GATE: Graph Attention Transformer Encoder for Cross-lingual Relation and Event Extraction

Recent progress in cross-lingual relation and event extraction use graph convolutional networks (GCNs) with universal dependency parses to learn language-agnostic sentence representations such that models trained on one language can be applied to other languages. However, GCNs struggle to model words with long-range dependencies or are not directly connected in the dependency tree. To address these challenges, we propose to utilize the self-attention mechanism where we explicitly fuse structural information to learn the dependencies between words with different syntactic distances. We introduce GATE, a {\bf G}raph {\bf A}ttention {\bf T}ransformer {\bf E}ncoder, and test its cross-lingual transferability on relation and event extraction tasks. We perform experiments on the ACE05 dataset that includes three typologically different languages: English, Chinese, and Arabic. The evaluation results show that GATE outperforms three recently proposed methods by a large margin. Our detailed analysis reveals that due to the reliance on syntactic dependencies, GATE produces robust representations that facilitate transfer across languages.

==> main_table/event_main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
% \resizebox{\linewidth}{!}{%
% \small
\begin{tabular}{l|c|c c c}
\hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{Source Language} & \multicolumn{3}{c}{Target Language} \\ 
\cline{3-5}
& & English & Chinese & Arabic \\ 
\hline
\multirow{6}{*}{\citet{liu2019neural}} & English & - & 32.5 & 51.3  \\
&  Chinese & 33.1 & - & 46.8  \\
&  Arabic & 32.4 & 28.0 & -  \\
\cline{2-5}
&  English + Chinese & - & - & 50.5 \\
&  English + Arabic & - & 32.5 & -  \\
&  Chinese + Arabic & 36.2 & - & - \\
\hline
\multirow{6}{*}{\citet{subburathinam2019cross}} & English & - & 44.4 & 45.9  \\
&  Chinese & 40.1 & - & 41.5  \\
&  Arabic & 29.0 & 39.1 & -  \\
\cline{2-5}
&  English + Chinese & - & - & 51.5 \\
&  English + Arabic & - & 51.3 & -  \\
&  Chinese + Arabic & 40.5 & - & - \\
\hline
\multirow{6}{*}{\citet{florian2019neural}} & English & - & 52.9 & 43.0  \\
&  Chinese & 46.1 & - & 40.4  \\
&  Arabic & 41.3 & 44.5 & -  \\
\cline{2-5}
&  English + Chinese & - & - & 48.9 \\
&  English + Arabic & - & 54.1 & -  \\
&  Chinese + Arabic & 51.7 & - & - \\
\hline
\multirow{6}{*}{GATE (This work)} & English & - & \textbf{57.1} & \textbf{54.8} \\
&  Chinese & \textbf{51.3} & - & \textbf{59.4}  \\
&  Arabic & \textbf{46.8} & \textbf{49.7} & -  \\
\cline{2-5}
&  English + Chinese & - & - & \textbf{60.1} \\
&  English + Arabic & - & \textbf{58.2} & -  \\
&  Chinese + Arabic & \textbf{55.3} & - & - \\
\hline
\end{tabular}
% }
\caption{
Event-Argument Role Labeling \emph{transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect event triggers.
In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
}
% }
\label{table:event_results}
% \vspace{-2mm}
\end{table*}


==> main_table/gate_vs_trans.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
% \resizebox{0.95\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c c c c c c|c c c c c c}
\hline
\multirow{4}{*}{Model} & \multicolumn{6}{c|}{Event Argument Role Labeling} & \multicolumn{6}{c}{Relation Extraction} \\
\cline{2-7}\cline{8-13}
& En & En & Zh & Zh & Ar & Ar & En & En & Zh & Zh & Ar & Ar \\ 
& $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ \\
& Zh & Ar & En & Ar & En & Zh & Zh & Ar & En & Ar & En & Zh \\ 
\hline
\multirow{1}{*}{\citet{vaswani2017attention}} & 61.5 & 55.0 & 58.0 & 57.7 & 54.3 & 57.0 & 57.1 & 63.4 & 69.6 & 60.6 & 67.0 & 52.6 \\
\multirow{1}{*}{Shaw et al. (2018)} & 62.3 & 60.8 & 57.3 & 66.3 & \textbf{57.5} & \textbf{59.8} & \textbf{58.0} & 59.9 & 70.0 & 55.6 & 66.5 & \textbf{56.5} \\
\multirow{1}{*}{GATE} & \textbf{63.2} & \textbf{68.5} & \textbf{59.3} & \textbf{69.2} & 53.9 & 57.8 & {55.1} & \textbf{66.8} & \textbf{71.5} & \textbf{61.2} & \textbf{69.0} & 54.3\\
\hline
\end{tabular}
% }
\vspace{-2mm}
\caption{
Single-source transfer results (F-score \% on the test set) using perfect event triggers and entity mentions.
% En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
The language on top and bottom of $\Downarrow$ denotes the source and target languages, respectively.
}
\label{table:gate_vs_trans}
\vspace{-2mm}
\end{table*}



==> main_table/main_result.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
% \resizebox{1.0\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c|c c c|c c c}
\hline
\multirowcell{3}{Model} & \multirowcell{3}{Source \\ Language} & \multicolumn{3}{c|}{EARL} & \multicolumn{3}{c}{RE} \\ 
\cline{3-8}
& & \multicolumn{6}{c}{Transfer Language} \\ 
\cline{3-8}
& & En & Zh & Ar & En & Zh & Ar \\ 
\hline
\multicolumn{7}{l}{{\bf Single-source Transfer (SST)}} \\
\hline
\multirowcell{3}{Baseline1. \\\cite{liu2019neural}} & En & - & 32.5 & 51.3 & - & 34.0 & 45.3 \\
& Zh & 33.1 & - & 46.8 & 49.2 & - & 39.6 \\
& Ar & 32.4 & 28.0 & - & 51.6 & 30.3 & - \\
\hline
\multirowcell{3}{Baseline2. \\\cite{subburathinam2019cross}} & En & - & 44.4 & 45.9 & - & 49.4 & 58.3 \\
& Zh & 40.1 & - & 41.5 & 65.0 & - & 55.0 \\
& Ar & 29.0 & 39.1 & - & 56.7 & 42.4 & - \\
\hline
\multirowcell{3}{Baseline3. \\\cite{florian2019neural}} & En & - & 52.9 & 43.0 & - & 53.7 & 63.9 \\
& Zh & 46.1 & - & 40.4 & 70.9 & - & 57.6 \\
& Ar & 41.3 & 44.5 & - & 67.1 & \textbf{55.7} & - \\
\hline
\multirowcell{3}{GATE \\(This work)} & En & - & \textbf{57.1} & \textbf{54.8} & - & \textbf{55.1} & \textbf{66.8} \\
& Zh & \textbf{51.3} & - & \textbf{59.4} & \textbf{71.5} & - & \textbf{61.2} \\
& Ar & \textbf{46.8} & \textbf{49.7} & - & \textbf{69.0} & 54.3 & - \\
\hline
\multicolumn{7}{l}{{\bf Multi-source Transfer (MST)}} \\
\hline
\multirowcell{3}{Baseline1. \\\cite{liu2019neural}} & En + Zh & - & - & 50.5 & - & - & 47.7 \\
& En + Ar & - & 32.5 & - & - & 33.1 & - \\
& Zh + Ar & 36.2 & - & - & 50.7 & - & - \\
\hline
\multirowcell{3}{Baseline2. \\\cite{subburathinam2019cross}} & En + Zh & - & - & 51.5 & - & - & 64.0 \\
& En + Ar & - & 51.3 & - & - & 46.6 & - \\
& Zh + Ar & 40.5 & - & - & 65.8 & - & - \\
\hline
\multirowcell{3}{Baseline3. \\\cite{florian2019neural}} & En + Zh & - & - & 48.9 & - & - & 66.5 \\
& En + Ar & - & 54.1 & - & - & \textbf{60.5} & - \\
& Zh + Ar & 51.7 & - & - & 73.0 & - & - \\
\hline
\multirowcell{3}{GATE \\(This work)} & En + Zh & - & - & \textbf{60.1} & - & - & \textbf{67.0} \\
& En + Ar & - & \textbf{58.2} & - & - & 57.9 & -  \\
& Zh + Ar & \textbf{55.3} & - & - & \textbf{74.1} & - & - \\
\hline
\end{tabular}
% }
\vspace{-2mm}
\caption{
Event Argument Role Labeling (EARL) and Relation Extraction (RE) \emph{transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect event triggers and entity mentions.
% SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
The bold-faced values indicate the best performances across the board.
We trained all the models three times with different initializations and reported average scores.
}
\label{table:results}
\vspace{-2mm}
\end{table*}


==> main_table/main_result_v0.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
\resizebox{0.9\linewidth}{!}{%
\small
\def\arraystretch{1.1}%
\begin{tabular}{l|l|c c c|c c c}
\hline
\multirowcell{3}{Setting} & \multirow{3}{*}{Source Language} & \multicolumn{3}{c|}{Event-Argument Role Labeling} & \multicolumn{3}{c}{Relation Extraction} \\ 
\cline{3-8}
& & \multicolumn{6}{c}{Transfer Language} \\ 
\cline{3-8}
& & English & Chinese & Arabic & English & Chinese & Arabic \\ 
\hline
\multicolumn{7}{l}{{\bf Baseline1.} \citet{liu2019neural}} \\
\hline
\multirow{3}{*}{SST} & English & - & 32.5 & 51.3 & - & 34.0 & 45.3 \\
& Chinese & 33.1 & - & 46.8 & 49.2 & - & 39.6 \\
& Arabic & 32.4 & 28.0 & - & 51.6 & 30.3 & - \\
\hline
\multirow{3}{*}{MST} & English + Chinese & - & - & 50.5 & - & - & 47.7 \\
& English + Arabic & - & 32.5 & - & - & 33.1 & - \\
& Chinese + Arabic & 36.2 & - & - & 50.7 & - & - \\
\hline
\multicolumn{7}{l}{{\bf Baseline2.} \citet{subburathinam2019cross}} \\
\hline
\multirow{3}{*}{SST} & English & - & 44.4 & 45.9 & - & 49.4 & 58.3 \\
& Chinese & 40.1 & - & 41.5 & 65.0 & - & 55.0 \\
& Arabic & 29.0 & 39.1 & - & 56.7 & 42.4 & - \\
\hline
\multirow{3}{*}{MST} & English + Chinese & - & - & 51.5 & - & - & 64.0 \\
& English + Arabic & - & 51.3 & - & - & 46.6 & - \\
& Chinese + Arabic & 40.5 & - & - & 65.8 & - & - \\
\hline
\multicolumn{7}{l}{{\bf Baseline3.} \citet{florian2019neural}} \\
\hline
\multirow{3}{*}{SST} & English & - & 52.9 & 43.0 & - & 53.7 & 63.9 \\
& Chinese & 46.1 & - & 40.4 & 70.9 & - & 57.6 \\
& Arabic & 41.3 & 44.5 & - & 67.1 & \textbf{55.7} & - \\
\hline
\multirow{3}{*}{MST} & English + Chinese & - & - & 48.9 & - & - & 66.5 \\
& English + Arabic & - & 54.1 & - & - & \textbf{60.5} & - \\
& Chinese + Arabic & 51.7 & - & - & 73.0 & - & - \\
\hline
\multicolumn{7}{l}{ {\bf GATE (This work)} } \\
\hline
\multirow{3}{*}{SST} & English & - & \textbf{57.1} & \textbf{54.8} & - & \textbf{55.1} & \textbf{66.8} \\
& Chinese & \textbf{51.3} & - & \textbf{59.4} & \textbf{71.5} & - & \textbf{61.2} \\
& Arabic & \textbf{46.8} & \textbf{49.7} & - & \textbf{69.0} & 54.3 & - \\
\hline
\multirow{3}{*}{MST} & English + Chinese & - & - & \textbf{60.1} & - & - & \textbf{67.0} \\
& English + Arabic & - & \textbf{58.2} & - & - & 57.9 & -  \\
& Chinese + Arabic & \textbf{55.3} & - & - & \textbf{74.1} & - & - \\
\hline
\end{tabular}
}
\caption{
Event-Argument Role Labeling and Relation Extraction \emph{transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect event triggers and entity mentions.
SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
The bold-faced values indicate the best performances across the board.
We trained all the models three times with different initializations and reported average scores.
}
\label{table:results}
\vspace{-2mm}
\end{table*}


==> main_table/main_result_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{%
\small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c|c@{\hskip 0.35in} c@{\hskip 0.35in} c|c c c}
\hline
\multirowcell{2}{Model} & \multirowcell{2}{Target \\ Language} & \multicolumn{6}{c}{Source Language} \\ 
\cline{3-8}
& & En & Zh & Ar & En + Zh & En + Ar & Zh + Ar \\ 
\hline
\multicolumn{7}{l}{{Event Argument Role Labeling}} \\
\hline
\multirowcell{3}{Baseline1. \\\cite{liu2019neural}} & En & - & 33.1 & 32.4 & - & - & 36.2 \\
& Zh & 32.5 & - & 28.0 & - & 32.5 & - \\
& Ar & 51.3 & 46.8 & - & 50.5 & - & - \\
\hline
\multirowcell{3}{Baseline2. \\\cite{subburathinam2019cross}} & En & - & 40.1 & 29.0 & - & - & 40.5 \\
& Zh & 44.4 & - & 39.1 & - & 51.3 & - \\
& Ar & 45.9 & 41.5 & - & 51.5 & - & - \\
\hline
\multirowcell{3}{Baseline3. \\\cite{florian2019neural}} & En & - & 46.1 & 41.3 & - & - & 51.7 \\
& Zh & 52.9 & - & 44.5 & - & 54.1 & - \\
& Ar & 43.0 & 40.4 & - & 48.9 & - & - \\
\hline
\multirowcell{3}{GATE \\(This work)} & En & - & \textbf{51.3} & \textbf{46.8} & - & - & \textbf{55.3} \\
& Zh & \textbf{57.1} & - & \textbf{49.7} & - & \textbf{58.2} & - \\
& Ar & \textbf{54.8} & \textbf{59.4} & - & \textbf{60.1} & - & - \\
\hline
\multicolumn{7}{l}{{Relation Extraction}} \\
\hline
\multirowcell{3}{Baseline1. \\\cite{liu2019neural}} & En & - & 49.2 & 51.6 & - & - & 50.7 \\
& Zh & 34.0 & - & 30.3 & - & 33.1 & - \\
& Ar & 45.3 & 39.6 & - & 47.7 & - & - \\
\hline
\multirowcell{3}{Baseline2. \\\cite{subburathinam2019cross}} & En & - & 65.0 & 56.7 & - & - & 65.8 \\
& Zh & 49.4 & - & 42.4 & - & 46.6 & - \\
& Ar & 58.3 & 55.0 & 64.0 & - & - \\
\hline
\multirowcell{3}{Baseline3. \\\cite{florian2019neural}} & En & - & 70.9 & 67.1 & - & - & 73.0 \\
& Zh & 53.7 & - & \textbf{55.7} & - & \textbf{60.5} & - \\
& Ar & 63.9 & 57.6 & - & 66.5 & - & - \\
\hline
\multirowcell{3}{GATE \\(This work)} & En & - & \textbf{71.5} & \textbf{69.0} & - & - & \textbf{74.1} \\
& Zh & \textbf{55.1} & - & 54.3 & - & 57.9 & -  \\
& Ar & \textbf{66.8} & \textbf{61.2} & - & \textbf{67.0} & - & - \\
\hline
\end{tabular}
}
\caption{
Event-Argument Role Labeling (EARL) and Relation Extraction (RE) \emph{transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect event triggers and entity mentions.
En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
% SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
The bold-faced values indicate the best performances across the board.
We trained all the models three times with different initialization and reported average scores.
}
\label{table:results}
\vspace{-2mm}
\end{table*}


==> main_table/main_result_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\resizebox{0.85\linewidth}{!}{%
\small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c c c c c c}
\hline
\multirow{1}{*}{Model} & En $\Rightarrow$ Zh & En $\Rightarrow$ Ar & Zh $\Rightarrow$ En & Zh $\Rightarrow$ Ar & Ar $\Rightarrow$ En & Ar $\Rightarrow$ Zh \\ 
\hline
\multicolumn{5}{l}{{Event Argument Role Labeling}} \\
\hline
\multirow{1}{*}{CL\_Trans\_GCN} & 32.5 & 51.3 & 33.1 & 46.8 & 32.4 & 28.0 \\
\multirow{1}{*}{CL\_GCN} & 44.4 & 45.9 & 40.1 & 41.5 & 29.0 & 39.1 \\
\multirow{1}{*}{CL\_RNN} & 52.9 & 43.0 & 46.1 & 40.4 & 41.3 & 44.5 \\
\multirow{1}{*}{GATE} & \textbf{57.1} & \textbf{54.8} & \textbf{51.3} & \textbf{59.4} & \textbf{46.8} & \textbf{49.7} \\
\hline
\multicolumn{5}{l}{{Relation Extraction}} \\
\hline
\multirow{1}{*}{CL\_Trans\_GCN} & 34.0 & 45.3 & 49.2 & 39.6 & 51.6 & 30.3 \\
\multirow{1}{*}{CL\_GCN} & 49.4 & 58.3 & 65.0 & 55.0 & 56.7 & 42.4 \\
\multirow{1}{*}{CL\_RNN} & 53.7 & 63.9 & 70.9 & 57.6 & 67.1 & \textbf{55.7} \\
\multirow{1}{*}{GATE} & \textbf{55.1} & \textbf{66.8} & \textbf{71.5} & \textbf{61.2} & \textbf{69.0} & 54.3 \\
\hline
\end{tabular}
}
\caption{
Event Argument Role Labeling (EARL) and Relation Extraction (RE) \emph{single-source transfer} results (F-score \%) using perfect event triggers and entity mentions.
En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
In ``X $\Rightarrow$ Y'', X and Y denotes the source and target language, respectively.
% SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
% The bold-faced values indicate the best performances across the board.
}
\label{table:sst_results}
\vspace{-2mm}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}{%
\small
% \def\arraystretch{1.1}%
% \begin{tabular}{l|@{}c@{\hskip 0.05in} c@{\hskip 0.05in} c@{}}
\begin{tabular}{l|c c c}
\hline
\multirow{3}{*}{Model} & \{En, Zh\} & \{En, Ar\} & \{Zh, Ar\} \\
& $\Downarrow$ & $\Downarrow$ & $\Downarrow$ \\
& Ar & Zh & En \\ 
\hline
\multicolumn{4}{l}{{Event Argument Role Labeling}} \\
\hline
CL\_Trans\_GCN & 50.5 & 32.5 & 36.2 \\
CL\_GCN & 51.5 & 51.3 & 40.5 \\
CL\_RNN & 48.9 & 54.1 & 51.7 \\
GATE & \textbf{60.1} & \textbf{58.2} & \textbf{55.3} \\
\hline
\multicolumn{4}{l}{{Relation Extraction}} \\
\hline
CL\_Trans\_GCN & 47.7 & 33.1 & 50.7 \\
CL\_GCN & 64.0 & 46.6 & 65.8 \\
CL\_RNN & 66.5 & \textbf{60.5} & 73.0 \\
GATE & \textbf{67.0} & 57.9 & \textbf{74.1} \\
\hline
\end{tabular}
}
\caption{
Event Argument Role Labeling (EARL) and Relation Extraction (RE) \emph{multi-source transfer} results (F-score \%) using perfect event triggers and entity mentions.
En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
% SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
% The bold-faced values indicate the best performances across the board.
}
\label{table:mst_results}
\vspace{-2mm}
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \resizebox{1.0\linewidth}{!}{%
% % \small
% % \def\arraystretch{1.1}%
% \begin{tabular}{l|c|c c c}
% \hline
% \multirow{2}{*}{Model} & \multirowcell{2}{Source\\Language} & \multicolumn{3}{c}{Target Language} \\ 
% \cline{3-5}
% & & En & Zh & Ar \\ 
% \hline
% \multicolumn{5}{l}{{Event Argument Role Labeling}} \\
% \hline
% \multirow{3}{*}{CL\_Trans\_GCN} & En & - & 32.5 & 51.3 \\
% & Zh & 33.1 & - & 46.8  \\
% & Ar & 32.4 & 28.0 & - \\
% \hline
% \multirow{3}{*}{CL\_GCN} & En & - & 44.4 & 45.9 \\
% & Zh & 40.1 & - & 41.5  \\
% & Ar & 29.0 & 39.1 & - \\
% \hline
% \multirow{3}{*}{CL\_RNN} & En & - & 52.9 & 43.0 \\
% & Zh & 46.1 & - & 40.4 \\
% & Ar & 41.3 & 44.5 & - \\
% \hline
% \multirow{3}{*}{GATE} & En & - & \textbf{57.1} & \textbf{54.8}  \\
% & Zh & \textbf{51.3} & - & \textbf{59.4} \\
% & Ar & \textbf{46.8} & \textbf{49.7} & - \\
% \hline
% \multicolumn{5}{l}{{Relation Extraction}} \\
% \hline
% \multirow{3}{*}{CL\_Trans\_GCN} & En & - & 34.0 & 45.3 \\
% & Zh & 49.2 & - & 39.6 \\
% & Ar & 51.6 & 30.3 & - \\
% \hline
% \multirow{3}{*}{CL\_GCN} & En & - & 49.4 & 58.3 \\
% & Zh & 65.0 & - & 55.0 \\
% & Ar & 56.7 & 42.4 & - \\
% \hline
% \multirow{3}{*}{CL\_RNN} & En & - & 53.7 & 63.9 \\
% & Zh & 70.9 & - & 57.6 \\
% & Ar & 67.1 & \textbf{55.7} & - \\
% \hline
% \multirow{3}{*}{GATE} & En & - & \textbf{55.1} & \textbf{66.8} \\
% & Zh & \textbf{71.5} & - & \textbf{61.2} \\
% & Ar & \textbf{69.0} & 54.3 & - \\
% \hline
% \end{tabular}
% }
% \caption{
% Event-Argument Role Labeling (EARL) and Relation Extraction (RE) \emph{single-source transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect event triggers and entity mentions.
% En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
% % SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% % In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
% % The bold-faced values indicate the best performances across the board.
% }
% \label{table:sst_results}
% \vspace{-2mm}
% \end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% \begin{table*}[t]
% \centering
% \resizebox{0.7\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
% \begin{tabular}{l|c c c}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{3}{c}{Source $\rightarrow$ Target} \\ 
% \cline{2-4}
% & \{En, Zh\} $\rightarrow$ Ar & \{En, Ar\} $\rightarrow$ Zh & \{Zh, Ar\} $\rightarrow$ En \\ 
% \hline
% \multicolumn{4}{l}{{Event Argument Role Labeling}} \\
% \hline
% CL\_Trans\_GCN & 50.5 & 32.5 & 36.2 \\
% CL\_GCN & 51.5 & 51.3 & 40.5 \\
% CL\_RNN & 48.9 & 54.1 & 51.7 \\
% GATE & \textbf{60.1} & \textbf{58.2} & \textbf{55.3} \\
% \hline
% \multicolumn{4}{l}{{Relation Extraction}} \\
% \hline
% CL\_Trans\_GCN & 47.7 & 33.1 & 50.7 \\
% CL\_GCN & 64.0 & 46.6 & 65.8 \\
% CL\_RNN & 66.5 & \textbf{60.5} & 73.0 \\
% GATE & \textbf{67.0} & 57.9 & \textbf{74.1} \\
% \hline
% \end{tabular}
% }
% \caption{
% Event-Argument Role Labeling (EARL) and Relation Extraction (RE) \emph{multi-source transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect event triggers and entity mentions.
% En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
% % SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% % In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
% % The bold-faced values indicate the best performances across the board.
% }
% \label{table:mst_results}
% \vspace{-2mm}
% \end{table*}


==> main_table/main_result_v3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\resizebox{0.9\linewidth}{!}{%
\small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c@{\hskip 0.15in} c@{\hskip 0.15in} c@{\hskip 0.15in} c@{\hskip 0.15in} c@{\hskip 0.15in} c|c@{\hskip 0.15in} c@{\hskip 0.15in} c@{\hskip 0.15in} c@{\hskip 0.15in} c@{\hskip 0.15in} c}
\hline
% \multirow{1}{*}{Model} & En $\Rightarrow$ Zh & En $\Rightarrow$ Ar & Zh $\Rightarrow$ En & Zh $\Rightarrow$ Ar & Ar $\Rightarrow$ En & Ar $\Rightarrow$ Zh \\ 
\multirow{4}{*}{Model} & \multicolumn{6}{c|}{Event Argument Role Labeling} & \multicolumn{6}{c}{Relation Extraction} \\
\cline{2-7}\cline{8-13}
& En & En & Zh & Zh & Ar & Ar & En & En & Zh & Zh & Ar & Ar \\ 
& $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ & $\Downarrow$ \\
& Zh & Ar & En & Ar & En & Zh & Zh & Ar & En & Ar & En & Zh \\ 
\hline
\multirow{1}{*}{CL\_Trans\_GCN} & 32.5 & 51.3 & 33.1 & 46.8 & 32.4 & 28.0 & 34.0 & 45.3 & 49.2 & 39.6 & 51.6 & 30.3\\
\multirow{1}{*}{CL\_GCN} & 44.4 & 45.9 & 40.1 & 41.5 & 29.0 & 39.1 & 49.4 & 58.3 & 65.0 & 55.0 & 56.7 & 42.4\\
\multirow{1}{*}{CL\_RNN} & 52.9 & 43.0 & 46.1 & 40.4 & 41.3 & 44.5 & 53.7 & 63.9 & 70.9 & 57.6 & 67.1 & \textbf{55.7} \\
\multirow{1}{*}{GATE} & \textbf{57.1} & \textbf{54.8} & \textbf{51.3} & \textbf{59.4} & \textbf{46.8} & \textbf{49.7} & \textbf{55.1} & \textbf{66.8} & \textbf{71.5} & \textbf{61.2} & \textbf{69.0} & 54.3\\
\hline
\end{tabular}
}
\caption{
Single-source transfer results (F-score \% on the test set) using perfect event triggers and entity mentions.
% En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
The language on top and bottom of $\Downarrow$ denotes the source and target languages, respectively.
% SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
% The bold-faced values indicate the best performances across the board.
}
\label{table:sst_results}
\vspace{-2mm}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|@{\hskip 0.1in}c@{\hskip 0.1in} c@{\hskip 0.1in} c@{\hskip 0.1in}}
\hline
\multirow{3}{*}{Model} & \{En, Zh\} & \{En, Ar\} & \{Zh, Ar\} \\
& $\Downarrow$ & $\Downarrow$ & $\Downarrow$ \\
& Ar & Zh & En \\ 
\hline
\multicolumn{4}{l}{{Event Argument Role Labeling}} \\
\hline
CL\_Trans\_GCN & 50.5 & 32.5 & 36.2 \\
CL\_GCN & 51.5 & 51.3 & 40.5 \\
CL\_RNN & 48.9 & 54.1 & 51.7 \\
GATE & \textbf{60.1} & \textbf{58.2} & \textbf{55.3} \\
\hline
\multicolumn{4}{l}{{Relation Extraction}} \\
\hline
CL\_Trans\_GCN & 47.7 & 33.1 & 50.7 \\
CL\_GCN & 64.0 & 46.6 & 65.8 \\
CL\_RNN & 66.5 & \textbf{60.5} & 73.0 \\
GATE & \textbf{67.0} & 57.9 & \textbf{74.1} \\
\hline
\end{tabular}
}
\caption{
Multi-source transfer results (F-score \% on the test set) using perfect event triggers and entity mentions.
The language on top and bottom of $\Downarrow$ denotes the source and target languages, respectively.
% En, Zh, and Ar denotes English, Chinese, and Arabic languages, respectively.
% SST and MST denotes the single-source transfer and multi-source transfer setting, respectively.
% In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
% The bold-faced values indicate the best performances across the board.
}
\label{table:mst_results}
\vspace{-2mm}
\end{table}





==> main_table/relation_main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
% \resizebox{\linewidth}{!}{%
% \small
\begin{tabular}{l|c|c c c}
\hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{Source Language} & \multicolumn{3}{c}{Target Language} \\ 
\cline{3-5}
& & English & Chinese & Arabic \\ 
\hline
\multirow{6}{*}{\citet{liu2019neural}} & English & - & 34.0 & 45.3 \\
&  Chinese & 49.2 & - & 39.6  \\
&  Arabic & 51.6 & 30.3 & -  \\
\cline{2-5}
&  English + Chinese & - & - & 47.7 \\
&  English + Arabic & - & 33.1 & -  \\
&  Chinese + Arabic & 50.7 & - & - \\
\hline
\multirow{6}{*}{\citet{subburathinam2019cross}} & English & - & 49.4 & 58.3 \\
&  Chinese & 65.0 & - & 55.0  \\
&  Arabic & 56.7 & 42.4 & -  \\
\cline{2-5}
&  English + Chinese & - & - & 64.0 \\
&  English + Arabic & - & 46.6 & -  \\
&  Chinese + Arabic & 65.8 & - & - \\
\hline
\multirow{6}{*}{\citet{florian2019neural}} & English & - & 53.7 & 63.9 \\
&  Chinese & 70.9 & - & 57.6  \\
&  Arabic & 67.1 & \textbf{55.7} & -  \\
\cline{2-5}
&  English + Chinese & - & - & 66.5 \\
&  English + Arabic & - & \textbf{60.5} & -  \\
&  Chinese + Arabic & 73.0 & - & - \\
\hline
\multirow{6}{*}{GATE (This work)} & English & - & \textbf{55.1} & \textbf{66.8} \\
&  Chinese & \textbf{71.5} & - & \textbf{61.2}  \\
&  Arabic & \textbf{69.0} & 54.3 & -  \\
\cline{2-5}
&  English + Chinese & - & - & \textbf{67.0} \\
&  English + Arabic & - & 57.9 & -  \\
&  Chinese + Arabic & \textbf{74.1} & - & - \\
\hline
\end{tabular}
% }
\caption{
Relation Extraction \emph{transfer} results (F-score \%) of our proposed approach and the baseline methods using perfect entity mentions.
In \citet{liu2019neural}, we use multilingual word embeddings \cite{joulin-etal-2018-loss}, while in other baselines and our approach, we use multilingual BERT \cite{devlin-etal-2019-bert} representations.
}
% }
\label{table:relation_results}
% \vspace{-2mm}
\end{table*}

